TRAP: Targeted Random Adversarial Prompt Honeypot for Black-Box Identification

Large Language Model (LLM) services and models often come with legal rules on who can use them and how they must use them. Assessing the compliance of the released LLMs is crucial, as these rules protect the interests of the LLM contributor and prevent misuse. In this context, we describe the novel fingerprinting problem of Black-box Identity Verification (BBIV). The goal is to determine whether a third-party application uses a certain LLM through its chat function. We propose a method called Targeted Random Adversarial Prompt (TRAP) that identifies the specific LLM in use. We repurpose adversarial suffixes, originally proposed for jailbreaking, to get a pre-defined answer from the target LLM, while other models give random answers. TRAP detects the target LLMs with over 95% true positive rate at under 0.2% false positive rate even after a single interaction. TRAP remains effective even if the LLM has minor changes that do not significantly alter the original function.

==> latex/bin.tex <==
% ***** BIN for old texts ******

% --- related ---


% \paragraph{LLM detection.} Detection of LLMs-generated text is a non-trivial task, as exemplified by studies like \citet{jannai_human_2023, jones_does_2023}.
% Several lines of research have investigated the effective detection of LLMs, including, for instance, \emph{watermarking} \citep{abdelnabi2021adversarial, kirchenbauer2023watermark, hu2023unbiased} --- the use of humanly imperceptible generation patterns that nonetheless allow for statistical detection of LLM authorship, exploiting properties of a model's probability space \citep{mitchell2023detectGPT}, analysing the text's statistical properties \citep{gehrmann2019gltr}, or directly training classifiers \citep{chen_gpt-sentinel_2023}.
% However, \citet{sadasivan2023can} show that these detectors are not reliable, and can e.g.\@ be spoofed by paraphrasing attacks.
% \citet{chakraborty2023possibilities} argue that as LLMs achieve text generation similar to humans, detection remains possible, albeit under a larger sample size of generated text.
% A more comprehensive overview of available methods is given by the surveys by \citet{dhaini2023detecting, ghosal2023towards}.
% - list of detecting LLMs papers: https://github.com/Xianjun-Yang/Awesome_papers_on_LLMs_detection
% - survey about LLM detection: https://twitter.com/amritsinghbedi3/status/1717039417540391205/photo/1 
% - survey a bit older: https://arxiv.org/abs/2309.07689
% - \citet{yang_anatomy_2023} detect artifact strings produced by aligned LLM, such as ``As an AI, I don't''. 


%Detecting LLM in interactive setups

%The development of LLMs is tightly linked to chatbot (conversational agent). Recent LLMs are designed to behave as conversational agents. OpenAI develops and distributes gpt-3.5-turbo for chat. Llama-2-Chat has been fine-tuned and optimized for dialogue use cases. 
%Nevertheless, the vast majority of LLM detectors behave in a static (non-interactive) manner. \citet{ghosal_towards_2023} claims that "it may be relatively easier to identify AI-generated text in an online interaction with AI agents", it remains speculative, since no evaluation on the topic, except \citet{wang_bot_2023}.
% The collection of additional samples is at the center of the controversy related to the feasibility/impossibility to detect LLM \citep{ghosal_towards_2023}.

% \paragraph{Attack against alignment.} The alignment problem constitutes the challenge of harmonizing LLMs' outputs with human goals and values \citep{yudkowsky2016ai, christian2020alignment}.
% This goal is currently being achieved by means of reinforcement learning from human feedback \citep{christiano2017deep, ziegler2019fine}, direct preference optimization \citep{rafailov2023direct}, distillation \citep{tunstall2023zephyr} and more (see \citet{fernandes2023bridging} for a survey of research teaching models to follow human feedback).
% However, plentiful ways to circumvent the alignment safety measures have been discovered as well:
% \citet{zou_universal_2023, liu2023autodan} automatically craft problems that trigger undesirable behaviours even after alignment, \citet{wei2023jailbreak} demonstrate the use of in-context examples for jailbreaking, while \citet{huang2023catastrophic} illustrate the impact of varying the generation methods.
% \citet{wolf2023fundamental} provide a theoretical framework and conclude that any alignment techniques that do not remove an undesired behaviour will always be prone to adversarial prompting attacks.
% - reverse-engineering the generation strategy (top-k or nucleus samping). "Prior work has shown that knowing the decoding method makes it easier to detect whether a writing sample was generated by a language model or else was human-written (Ippolito et al., 2020)". https://arxiv.org/pdf/2309.04858.pdf 
% - summary thread of recent papers showing how brittle alignment is: https://twitter.com/amritsinghbedi3/status/1717039417540391205
% - Just a few in-context demonstrations is enough to jailbreak. Without adversarial suffix. https://arxiv.org/pdf/2310.06387.pdf
% - Related work on representation learning and alignment when faced with adversarial suffixes  https://twitter.com/DanHendrycks/status/1709227490592612671
% - Jailbreaking (white-box; ie, open-sourced) LLMs by manipulating decoding hyper-parameter: https://princeton-sysml.github.io/jailbreak-llm/

% Adversarial suffixes can be optimized to force the LLM to output an answer chosen at random. \citet{zou_universal_2023} propose Greedy Coordinate Gradient (GCG) to find prompt suffixes that jailbreak the alignment of LLMs. GCG finds the suffix tokens that minimize the loss of strings that are the beginning of a positive answer, like ``Sure, here's a''. 





% --- motivation ---

\section{Motivation}

Detecting LLM in interactive setups

\subsection{Turing Test}
Turing test: a \textit{human} is trying to distinguish between another human and an LLM.

We need to motivate the existence of such a tool. Motivation question: can a human recognize a chatbot from another human without any tool? \citet{jannai_human_2023} \citet{jones_does_2023}...

The development of LLMs is tightly linked to chatbot (conversational agent). Recent LLMs are designed to behave as conversational agents. OpenAI develops and distributes gpt-3.5-turbo for chat. Llama-2-Chat has been fine-tuned and optimized for dialogue use cases. 

Nevertheless, the vast majority of LLM detectors behave in a static (non-interactive) manner. \citet{ghosal_towards_2023} claims that "it may be relatively easier to identify AI-generated text in an online interaction with AI agents", it remains speculative, since no evaluation on the topic, except \citet{wang_bot_2023}.

The collection of additional samples is at the center of the controversy related to the feasibility/impossibility to detect LLM \citep{ghosal_towards_2023}.

\textbf{TODO 2.} If motivation 1 holds. Then: can we design simpler tools to detect LLM than adv suffix. Ex: obtain the distribution of random numbers/words for each LLM --> if similar, then LLM detected.
Two limitations:
1. may require many samples -> a human would not give 50 random numbers. Depend on how unique are the reply of LLMs
2. this simpler solution may not be robust to some minor changes. Ex: change in system prompt "you love animal and only talk about that" -> reply with animal names only when asked  random words. 


\subsection{Reverse Turing Test: Captcha for LLM}
%OTHER possibility:
Propose a new Captcha. Reverse Turing test: a \textit{machine} is trying to distinguish between another human and a LLM

% captcha or honeypot

Scenario: 
- an LLM/or a message/request/etc.
- the (customer/technical) support wants to ensure that the person is real before investing time in the request
- the human/LLM has to fill our "captcha" before continuing

\textbf{Issue:} The Captcha works as long as it is not removed/filtered.


% Note:
% - more use cases on https://kai-greshake.de/posts/in-escalating-order-of-stupidity/ ?



% --- TRAP ---


% First, we show that optimizing the tokens of the suffix following a question can reliably force the LLM to a specific answer. Second, we show that the found suffix does not transfer to other LLM, and can therefore identify a specific LLM. Third, we establish that these suffixes are robust to changes in the generation hyperparameters and to changes in system prompts. 




% A model different from the reference model is expected to follow the base instruction and sample the answer randomly from a pool of 
% For each suffix, a targeted answer is sampled uniformly at random, i.e., the target is a random number composed of $N$ digits. We apply GCG to select the suffix tokens that minimize the loss of the string ``Sure, here is a random string of N digits: XXXX'', where \verb|XXXX| is the targeted number. To ensure that the suffix does not encode straightforwardly the targeted number, we filter tokens that correspond to digits or to words that relate to digits.


% Adversarial suffixes can be optimised to force the LLM to output an answer chosen at random. \citet{zou_universal_2023} propose Greedy Coordinate Gradient (GCG) to find prompt suffixes that jailbreak the alignment of LLMs. GCG finds the suffix tokens that minimize the loss of strings that are the beginning of a positive answer, like ``Sure, here's a''. 

% We repurpose GCG to optimise a suffix that would force the model to output a specific answer to a question. Specifically, we ask the model to generate a random number, using the following prompt: ``Write a random string composed of N digits.'', where $N$ is chosen by us. For each suffix, a targeted answer is sampled uniformly at random, i.e., the target is a random number composed of $N$ digits. We apply GCG to select the suffix tokens that minimize the loss of the string ``Sure, here is a random string of N digits: XXXX'', where \verb|XXXX| is the targeted number. To ensure that the suffix does not encode straightforwardly the targeted number, we filter tokens that correspond to digits or to words that relate to digits.


% Therefore, by prompting a suffix optimised for a specific answer, we can reliably get this answer by one model.   

% and the rate of targeted answers by a non-reference model


% \subsection{Identifying Specific LLMs}

% We find that suffixes can force an LLM into a specific answer. But to identify specifically an LLM, we also need the suffix to be successful only against one LLM. We first establish the specificity of suffixes. Then we analyze the error rates. And finally, we show that we can optimise one suffix to detect several models at once.


%Suffixes optimised on Vicuna-7B never (0\%) retrieve the targeted answer when fed to the other five models. 
%The same observation is valid for suffixes optimised on Llama-2-7B-chat, except for one of the 100 suffixes. This exception is likely due to the relationship between both models, since Guanaco-7B is fined-tuned from Llama-2-7B. 
%In addition, we evaluated our suffixes on independently trained black-box models. Specifically, we feed the 100 suffixes optimised on Llama-2-7B-chat to OpenAI's GPT 3.5 (\verb|gpt-3.5-turbo-1106|) and GPT 4 (\verb|gpt-4-0613|), and to Anthropic's Claude 2.1 and Claude Instant 1.2. We generated ten answers for every suffix on every evaluated model. 
%None corresponds to the targeted number used to optimise the suffix. 
% Therefore, a suffix can uniquely identify an LLM, since it does not retrieve the targeted answer when fed to another independently trained LLM.

%The suffixes optimised on both Vicuna-7B and Guanaco-7B can reliably detect these two models, retrieving the target answer at least 81\% of the time. These suffixes do not retrieve the answer on other models. Similarly to the suffixes optimised on a single model, the suffixes do not retrieve the targeted answer on the OpenAI's GPT 3.5 and GPT 4 and Anthropic's Claude 2.1 and Claude Instant 1.2 models. Overall, suffixes can be optimised on an ensemble of models to detect more than one model.

% , ordered by difficulty and cost
% , in the weights after partial and full parameter fine-tuning


%\begin{figure}[htbp]
%  \centering
%  \begin{subfigure}{0.5\columnwidth}
%      \centering
%      \includegraphics[width=\linewidth]{fig/plot_temperature.pdf}
%      \caption{Temperature}
%      \label{fig:hp-temperature}
%  \end{subfigure}%
%  %\hfill
%  \begin{subfigure}{0.5\columnwidth}
%      \centering
%      \includegraphics[width=\linewidth]{fig/plot_top_p.pdf}
%      \caption{Top-p}
%      \label{fig:hp-top-p}
%  \end{subfigure}
%  \caption{Sensitivity to the generation hyperparameters. The x-axis indicates the hyperparameter value used to generate answers to each suffix. Evaluation of 100 suffixes created for the Llama-2-7B-chat model with the hyperparameter marked by the yellow vertical bar.}
%  \label{fig:generation-hps}
%\end{figure}






%----
ensemble multiple models 

When optimized on more models, the suffix starts to transfer to other models of the same family. The suffixes optimized on the ensemble of Vicuna-7B, Guanaco-7B, LLama2-7B-chat and Wizard-7B do retrieve the correct answer 5.6\% and 1.3\% of the time on respectively Vicuna-13B and Guanaco-13B. Nevertheless, these suffixes are never successful on GPT 3.5, GPT 4, Claude 2.1 and Claude Instant 1.2 models. 

% ------------
% Conclusion

% This behaviour can identify whether an unidentified LLM corresponds to a specific set of LLM weights. Identifying the deployed LLM to power a third-party service is relevant to detecting unauthorized usages of both open and closed source LLMs.

% Our technique is relevant for both use cases, since we can identify a specific LLM reliably with a very low false positive rate in very few queries. A very low false positive rate is at upmost importance in the cases motivated above. Indeed, LLM providers preparing for a judicial trial need strong evidence that they did not misidentify their LLM in an illegal situation.

% Our experiments also reveal the expressivity of LLM's input-output dependence, and the non-humanly interpretable correlations learned by LLMs. A prompt suffix can force the LLM to output an arbitrary answer, despite containing no human understandable ways to encode the specific answer. In our study, we restrict the candidate tokens in the suffix to contain no digits nor words that relate to numbers. Despite this limitation, we found suffixes that can reliably force the LLM to output a specific randomly selected number. To the human eye, these suffixes do not encode numbers, but somehow an LLM correlates these suffixes with specific numbers. Therefore, LLM learned strong correlations that end up in strong input-output dependencies. These correlations may be spurious, or grounded but not understandable for humans. Memorized training data can fit in this last case and induce strong dependencies. 

%For example, the token temperature in input can induce a specific memorized temperature, or some programming syntax may be associated with specific memorized numbers. 


\paragraph{Limitations and threat to validity}

- the adv suffix could contain indications that a human could parse and understand. Despite our best attempt at filtering tokens related to numbers, some suffix might encode part of the number (for example: XXXX for 4). In a real scenario, a safe way could be to check the produce suffix to ensure no human-understandable encoding is included. TODO: XP where we give our prompt+suffixes to real human?

% --------

Motivation. Answer w/o suffix

Even when generation hyperparameters are set to sample with very high diversity (sampling with very high temperature, such as 2.0 and top-p nucleus sampling of 1.0). Llama-2-7B has more diversity, but the distribution is still very much concentrated, since the most frequent number is sampled 56\% of the time. Models answers remain very concentrated even for high temperature (see Figure XX). This concentration means that model leave fingerprinted answers. 


Naive prompting intro

%Naive prompting cannot reliably identify an LLM due to unreliable answers and the ease of deception through system prompts. 
%These issues highlight the need for more advanced identification techniques beyond simple inquiries about the model's identity.

==> tab/results_system_prompts.tex <==
\begin{table}[tb]

\caption{Robustness of suffixes to different system prompts. Retrieval rates of 100 suffixes optimized on Llama-2-7B-chat using the default system prompts and evaluated on different system prompts. The answers are four digits long.}
\centering

\begin{tabular}{@{}p{0.47\linewidth}p{0.2\linewidth}p{0.23\linewidth}@{}}
\toprule
System Prompt                 & Retrieval Rate & No Answer Rate \\ \midrule
Default Llama-2               &  95.74 \%      &    01.30 \%     \\
Default OpenAI                &  45.12 \%      &    01.60 \%    \\
Default FastChat              &  65.12 \%      &    03.10 \%            \\
Shakespeare writing assistant &  18.97 \%      &    68.90 \%    \\
IRS tax assistant             &  25.46 \%      &    07.30 \%     \\
Marketing writing assistant   &  60.06 \%      &    03.10 \%    \\
Xbox customer support agent   &  57.14 \%      &    04.10 \%    \\
Hiking recommendation chatbot &  39.89 \%      &    05.50 \%    \\
JSON formatter assistant      &  57.31 \%      &    03.50 \%   \\ \bottomrule
\end{tabular}

\label{tab:results-system-prompt}
\end{table}



==> tab/results_transferability_opensource.tex <==
\begin{table*}[tb]

\caption{\small\textbf{Specificity of TRAP.} Suffixes uniquely identify a model. Confusion matrix of retrieval rates of 100 suffixes optimized on models in rows and evaluated on the model in columns. The answers are four digits long. In \%.} % Evaluation on other black-box models are available in supplementary materials.
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[t]{p{0.31\linewidth}rrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Retrieval Rate (\%)} \\
\cmidrule(l{3pt}r{3pt}){2-7}
Optimized on & Vicuna-7B & Vicuna-13B & Guanaco-7B & Guanaco-13B & Llama2-7B-chat & Llama2-13B-chat\\
\midrule
Vicuna-7B & 97.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
Vicuna-7B + Guanaco-7B & 84.8 & 0.0 & 81.8 & 0.0 & 0.0 & 0.0\\
Vicuna-7B + Guanaco-7B \newline + LLama2-7B-chat + Wizard-7B & 50.6 & 1.3 & 54.6 & 5.6 & 25.1 & 0.0\\
Llama2-7B-chat & 0.0 & 0.0 & 1.0 & 0.0 & 95 & 0.0\\
\bottomrule
\end{tabular}
\label{tab:results-transferability}
}
\end{table*}



==> tab/tab_example.tex <==
\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{ACL only command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| &  \\
\citealp{Gusfield:97} & \verb|\citealp| & \\
\citet{Gusfield:97} & \verb|\citet| &  \\
  \citeyearpar{Gusfield:97} & \verb|\citeyearpar| &  \\
  \citeposs{Gusfield:97}	&	& \verb|\citeposs|\\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}



\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

